A BiRGAT Model for Multi-intent Spoken Language Understanding with Hierarchical Semantic Frames

Previous work on spoken language understanding (SLU) mainly focuses on single-intent settings, where each input utterance merely contains one user intent. This configuration significantly limits the surface form of user utterances and the capacity of output semantics. In this work, we first propose a Multi-Intent dataset which is collected from a realistic in-Vehicle dialogue System, called MIVS. The target semantic frame is organized in a 3-layer hierarchical structure to tackle the alignment and assignment problems in multi-intent cases. Accordingly, we devise a BiRGAT model to encode the hierarchy of ontology items, the backbone of which is a dual relational graph attention network. Coupled with the 3-way pointer-generator decoder, our method outperforms traditional sequence labeling and classification-based schemes by a large margin.

==> 5.related.tex <==
\section{Related Work}
\paragraph{Multi-intent SLU}
It extends the classic single-intent setting, based on the fact that users often make multiple requests in one utterance. To deal with this generic scenario, existing models can be classified into four categories: 1) The first method treats each combination of multiple intents as a single intent label~\cite{shared-mi}. In this way, the multi-intent detection is reduced to single-intent case. However, it suffers from the label sparsity problem especially with the increase of intent number. 2) The second branch directly refines the original multi-class intent detection into multi-label sentence classification~\cite{joint-mi}. The output module needs to determine the feasibility of each intent individually. Though simple, it can not handle the aforementioned slot-intent assignment problem. 3) The third one firstly splits the input utterance into sub-sentences~\cite{two-stage}. The basic assumption is that each sub-sentence exactly represents one single intent. Next, a single-intent SLU model parses each sub-sentence and the outputs are merged via post-processing. The splitting criterion can be heuristic rules such as finding the conjunction words~(e.g., ``and''). Unfortunately, the user input may be too casual to be well-partitioned. 4) Another scheme transforms the output structure into a flattened sequence and utilizes a generator to produce the tokens one-by-one~\cite{topv2}. In this work, we adapt this method with a three-way copy mechanism to ensure the validity of output sequence on our newly proposed Chinese multi-domain multi-intent dataset MIVS.

\paragraph{Ontology Encoding for SLU}
Instead of initializing the weights of output labels randomly, \citet{label-zero} leverages BERT to encode intents. \citet{labelembed} extends the idea of label embeddings and integrates the text description, slot values and question exemplars to obtain the features of each slot label. \citet{hou2020few} further exploits label semantics in few-shot cross-domain settings.
To address the correlation between intents and slots, previous work introduces structural biases into model design. Both Slot-Gate~\cite{slot-gate} and Stack-Propagation~\cite{stackprop} utilize information from intents to control the prediction of slots. \citet{chen2020schema} constructs a schema graph among slots to inject inner relationships. Moreover, AGIF~\cite{agif} and GL-GIN~\cite{gl-gin} append an intent-slot graph interaction layer to model the bidirectional dependencies between slots and intents.
In this work, we follow the above ideas of semantic encoding and structural modeling for ontology items, and generalize to more universal multi-domain cases. Both the text description and the hierarchy of domains, intents and slots are taken into account.

==> tabs/mivs.tex <==
% Table generated by Excel2LaTeX from sheet 'mivs'
\begin{table*}[htbp]
  \centering
  \resizebox{0.98\textwidth}{!}{
    \begin{tabular}{l|l}
    \hline

    \hline
    \textbf{Input} & Play the song JANE \\\hdashline
    \textbf{Output} & \makecell[l]{(json) [\{`domain': `music', `intents': [\{`intent': `play music', `slots': \\\qquad[\{`slot': `act', `value': `play'\}, \{`slot': `target', `value': `song'\}, \{`slot': `song name', `value': `JANE'\}]\}]\}]}\\\hdashline
    \textbf{Serialized} & \{ \colorbox{domaincolor}{music} [ \colorbox{intentcolor}{play music} ( \colorbox{slotcolor}{act} = \colorbox{wordcolor}{play} ) ( \colorbox{slotcolor}{target} = \colorbox{wordcolor}{song} ) ( \colorbox{slotcolor}{song name} = \colorbox{wordcolor}{JANE} ) ] \} \\
    \hline
    \textbf{Input} & Open sunshade curtains and skylights \\\hdashline
    \textbf{Output} &  \makecell[l]{(json) [\{`domain': `in-vehicle control', `intents': [\{`intent': `car body control', `slots': [\{`slot': `act', `value': `open'\},\\\qquad\{`slot': `target', `value': `sunshade curtains'\}]\}, \{`intent': `car body control', `slots': \\\qquad\qquad[\{`slot': `act', `value': `open'\}, \{`slot': `target', `value': 'skylights'\}]\}]\}]} \\\hdashline
    \textbf{Serialized} & \makecell[l]{\{ \colorbox{domaincolor}{in-vehicle control} [ \colorbox{intentcolor}{car body control} ( \colorbox{slotcolor}{act} = \colorbox{wordcolor}{open} ) ( \colorbox{slotcolor}{target} = \colorbox{wordcolor}{sunshade curtains} ) ] \\\qquad[ \colorbox{intentcolor}{car body control} ( \colorbox{slotcolor}{act} = \colorbox{wordcolor}{open} ) ( \colorbox{slotcolor}{target} = \colorbox{wordcolor}{skylights} ) ] \}} \\
    \hline
    \textbf{Input} & How is the weather today, by the way navigate to Changting Road \\\hdashline
    \textbf{Output} & \makecell[l]{(json)~[\{`domain': `weather', `intents': [\{`intent': `query about weather', \\\qquad`slots': [\{`slot': `act', `value': `request'\}, \{`slot': `date', `value': `today'\}, \{`slot': `target', `value': `weather'\}]\}]\}, \\\qquad\qquad\{`domain': `map', `intents': [\{`intent': `navigation', `slots': [\{`slot': `destination', `value': `Changting Road'\}]\}]\}]}\\\hdashline
    \textbf{Serialized} & \makecell[l]{\{ \colorbox{domaincolor}{weather} [ \colorbox{intentcolor}{query about weather} ( \colorbox{slotcolor}{act} = \colorbox{wordcolor}{request} ) ( \colorbox{slotcolor}{date} = \colorbox{wordcolor}{today} ) ( \colorbox{slotcolor}{target} = \colorbox{wordcolor}{weather} ) ] \}\\\qquad\{ \colorbox{domaincolor}{map} [ \colorbox{intentcolor}{navigation} ( \colorbox{slotcolor}{destination} = \colorbox{wordcolor}{Changting Road} ) ] \}} \\
    \hline

    \hline
    \end{tabular}%
    }
  \caption{Single-intent, multi-intent and multi-domain examples~(from top to bottom) in MIVS dataset. We translate the original Chinese utterances and labels into English for clarity. The serialized format is indeed the output sequence $y$ of our decoder. Braces ``\{$\cdots$\}'', brackets ``[$\cdots$]'' and parentheses ``($\cdots$)'' function as sentinel guards for domain, intent and slot-value pair respectively.}
  \label{tab:mivs}%
\end{table*}%


==> tabs/prompt.tex <==
\begin{table*}[htbp]
    \centering
    \resizebox{0.98\textwidth}{!}{
    \begin{tabular}{l}
    \hline

    \hline
    The specification of ontology is defined as follows. \\
    Domain: map; \\
    Intents include: sys.cancel, navigation, peripheral search, $\cdots$ ;\\
    Slots include: \_\_act\_\_, \_\_tgt\_\_, destination name, destination type, $\cdots$;\\
    Domain: weather;\\
    Intents include: sys.cancel, query about city, query about weather, query about date, $\cdots$;\\
    Slots include: \_\_act\_\_, \_\_tgt\_\_, region, country, place, scene, city, $\cdots$;\\
    Domain: music;\\
    Intents include: sys.cancel, sys.select, sys.confirm, play music, $\cdots$;\\
    Slots include: \_\_act\_\_, \_\_tgt\_\_, theme, song name, year, rankings, $\cdots$;\\
    \quad\\
    Given the ontology, translate the input utterance into the output sequence. Please adhere to the output format.\\
    \quad\\
    Utterance: Please sing a song COOPERS LAST STAND ;\\
    Output: \{ music [ play music ( operation = sing ) ( song name = COOPERS LAST STAND ) ] \} ;\\
    \quad\\
    Utterance: How about the weather on September 1st ;\\
    Output: \{ weather [ query about weather ( \_\_act\_\_ = request ) ( date = September 1st ) ( \_\_tgt\_\_ = weather ) ] \} ;\\
    \quad\\
    $\cdots\cdots$\\
    \quad\\
    Utterance: I want to go to Qinghai Lake ;\\
    Output: \{ map [ navigation ( destination name = Qinghai Lake ) ] \} ;\\
    \quad\\
    Utterance: How about the weather and navigate to Shanghai ;\\
    Output: \\
    \hline

    \hline
    \end{tabular}
    }
    \caption{A translated prompting example from Chinese dataset MIVS. Due to space limit, intents and slots are truncated by symbol ``$\cdots$'', and more demonstration exemplars are truncated by symbol ``$\cdots\cdots$''. Notice that, the example above is evaluated under zero-shot settings and merely uses out-of-distribution exemplars. In other words, the prompting exemplars do not involve the domain combination ``{\it weather+map}'' that the test case focuses on.}
    \label{tab:llm+icl}
\end{table*}

==> tabs/rate.tex <==
% Table generated by Excel2LaTeX from sheet 'rate'
\begin{table}[htbp]
  \centering
    \begin{tabular}{c|ccc}
    \hline

    \hline
    \textbf{Method} & \textbf{SL} & \textbf{SL+CLF} & \textbf{Ours} \\
    \hline
    MIVS  &   48.1  &   80.6    & 100.0 \\
    TOPv2 &  75.3  & 84.3 & 99.6 \\
    \hline

    \hline
    \end{tabular}%
  \caption{Successful conversion rate of different decoding methods on dataset MIVS and TOPv2.}
  \label{tab:rate}%
\end{table}%


==> tabs/relation.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
  \centering
  \resizebox{0.98\textwidth}{!}{
    \begin{tabular}{c|c|c|l}
    \hline

    \hline
    \multicolumn{1}{c|}{\textbf{Relation} $z_{ij}$} & \multicolumn{1}{c|}{\textbf{Type of node} $i$} & \multicolumn{1}{c|}{\textbf{Type of node} $j$} & \textbf{Description} \\
    \hline
    \multirow{4}{*}{Self-loop} & \multicolumn{1}{c|}{\textsc{Domain}} & \multicolumn{1}{c|}{\textsc{Domain}} & Self-loop for domain $o_i$ \\
          & \multicolumn{1}{c|}{\textsc{Intent}} & \multicolumn{1}{c|}{\textsc{Intent}} & Self-loop for intent $o_i$ \\
          & \multicolumn{1}{c|}{\textsc{Slot}} & \multicolumn{1}{c|}{\textsc{Slot}} & Self-loop for slot $o_i$ \\
          & \multicolumn{1}{c|}{\textsc{Question}} & \multicolumn{1}{c|}{\textsc{Question}} & Self-loop for question word $q_i$ \\
    \hdashline
    Parent-of & \textsc{Domain} & \multicolumn{1}{c|}{\textsc{Intent}} & Domain $o_i$ is one parent of intent $o_j$ \\
    Grandparent-of &   \textsc{Domain}    & \multicolumn{1}{c|}{\textsc{Slot}} & Domain $o_i$ is one grandparent of slot $o_j$ \\
    Parent-of &   \textsc{Intent}    & \multicolumn{1}{c|}{\textsc{Slot}} & Intent $o_i$ is one parent of slot $o_j$ \\
    \hdashline
    Distance+1 & \multirow{4}{*}{\textsc{Question}} & \multirow{4}{*}{\textsc{Question}} & $q_j$ is the word to the right of $q_i$ \\
    Distance+2 &       &       & $q_j$ is the second word to the right of $q_i$ \\
    Distance+3 &       &       & $q_j$ is the third word to the right of $q_i$ \\
    Distance>3 &       &       & $q_j$ is the word to the right of $q_i$ with distance $>3$ \\
    \hline

    \hline
    \end{tabular}%
    }
  \caption{Relations $z_{ij}$ defined in this work according to the ontology hierarchy. For brevity, we only show one direction of an asymmetric relation~(the two blocks at the bottom), and the opposite can be easily inferred.}
  \label{tab:relation}%
\end{table*}%


==> tabs/topv2.tex <==
% Table generated by Excel2LaTeX from sheet 'topv2'
\begin{table*}[htbp]
  \centering
  \resizebox{0.98\textwidth}{!}{
    \begin{tabular}{l|l}
    \hline

    \hline
    \textbf{Input} & Set the alarm for tonight. \\
    \hdashline
    \textbf{Original} & [IN:CREATE\_ALARM Set the alarm [SL:DATE\_TIME for tonight ] . ] \\
    \hdashline
    \textbf{Converted} & \makecell[l]{
    (json) [\{`domain': `alarm', `intents': [\{`intent': `create alarm', \\\qquad `slots': [\{`slot': `date time', `value': `for tonight'\}]\}]\}]
    }\\\hdashline
    \textbf{Linearized} & \{ \colorbox{domaincolor}{alarm} [ \colorbox{intentcolor}{create alarm} ( \colorbox{slotcolor}{date time} = \colorbox{wordcolor}{for tonight} ) ] \}\\
    \hline
    \textbf{Input} & remove tomorrows alarms \\
    \hdashline
    \textbf{Original} & \makecell[l]{[IN:DELETE\_ALARM remove [SL:ALARM\_NAME [IN:GET\_TIME \\\qquad [SL:DATE\_TIME tomorrows ] ] ] alarms ]} \\
    \hdashline
    \textbf{Converted output} & \makecell[l]{(json) [\{`domain': `alarm', `intents': [\{`intent': `delete alarm', \\\qquad `slots': [\{`slot': `alarm name', `value': `tomorrows alarms'\}]\}, \\\qquad\{`intent': `get time', `slots': [\{`slot': `date time', `value': `tomorrows'\}]\}]\}]} \\
    \hdashline
    \textbf{Linearized} & \{ \colorbox{domaincolor}{alarm} [ \colorbox{intentcolor}{delete alarm} ( \colorbox{slotcolor}{alarm name} = \colorbox{wordcolor}{tomorrows alarms} ) ] [ \colorbox{intentcolor}{get time} ( \colorbox{slotcolor}{date time} = \colorbox{wordcolor}{tomorrows} ) ] \}\\
    \hline

    \hline
    \end{tabular}%
    }
  \caption{Examples of converting output labels for dataset TOPv2~\cite{topv2}.}
  \label{tab:topv2}%
\end{table*}%

